Asymptotic Privacy Loss due to Time Series Matching of Dependent Users

The Internet of Things (IoT) promises to improve user utility by tuning applications to user behavior, but revealing the characteristics of a user's behavior presents a significant privacy risk. Our previous work has established the challenging requirements for anonymization to protect users' privacy in a Bayesian setting in which we assume a powerful adversary who has perfect knowledge of the prior distribution for each user's behavior. However, even sophisticated adversaries do not often have such perfect knowledge; hence, in this paper, we turn our attention to an adversary who must learn user behavior from past data traces of limited length. We also assume there exists dependency between data traces of different users, and the data points of each user are drawn from a normal distribution. Results on the lengths of training sequences and data sequences that result in a loss of user privacy are presented.

==> outline_copy.tex <==




\section{Framework}
\label{frame}





\begin{thm}\label{IndependentCase}

\end{thm}

%\hspace{-0.14 in}\textbf{Discussion}:

%{\hspace{-0.18 in}\textbf{Discussion:}}





